Bayesian Deep Learning Hyperparameter Search for Robust Function Mapping to Polynomials with Noise

Advances in neural architecture search, as well as explainability and interpretability of connectionist architectures, have been reported in the recent literature. However, our understanding of how to design Bayesian Deep Learning (BDL) hyperparameters, specifically, the depth, width and ensemble size, for robust function mapping with uncertainty quantification, is still emerging. This paper attempts to further our understanding by mapping Bayesian connectionist representations to polynomials of different orders with varying noise types and ratios. We examine the noise-contaminated polynomials to search for the combination of hyperparameters that can extract the underlying polynomial signals while quantifying uncertainties based on the noise attributes. Specifically, we attempt to study the question that an appropriate neural architecture and ensemble configuration can be found to detect a signal of any n-th order polynomial contaminated with noise having different distributions and signal-to-noise (SNR) ratios and varying noise attributes. Our results suggest the possible existence of an optimal network depth as well as an optimal number of ensembles for prediction skills and uncertainty quantification, respectively. However, optimality is not discernible for width, even though the performance gain reduces with increasing width at high values of width. Our experiments and insights can be directional to understand theoretical properties of BDL representations and to design practical solutions.

==> removed.tex <==
\section{Background}

Recent successes [CITE papers] of ANNs, including MultiLayer Perceptrons (MLPs) and Deep Learning (DL) representations, have led to theoretical and empirical studies [CITE papers] to explore how hyperparameters such as depth and width impact the expressive capacity of neural networks. However, gaps remain in our understanding, including in deep learning [CITE PNAS paper]. The possible existence of an optimal depth in ANNs has received most attention in work related to ANN hyperparameter search. Such works~\cite{eldan2016power, cohen2016expressive, liang2016deep} shows the existence of certain deep ReLU networks that cannot be realized form shalllow networks. Zhou et al.~\cite{lu2017expressive} on the other hand, explores how width affects the expressiveness of neural networks and shows the existence of classes of wide networks which cannot be realized by any narrow network whose depth is no more than a polynomial bound. Poggio et al.~\cite{poggio2017and} provide theorems and examples of a class of compositional functions for which there is a gap between approximation in shallow and deep networks.

Theoretical papers on ANNs including MLPs and DL, have focused on performance guarantees often based on simplifying assumptions [CITE papers]. Practical papers have mostly dealt with searching for neural architectures that produce best prediction skills [CITE papers). However, what has received limited attention in the literature is the influence of hyperparameter selection on robust out-of-sample generalization and uncertainty characterization. One of the key challenges in the analysis of  generalization bounds in deep neural networks is that it may vary depending on the data distribution on which networks is trained. Therefore, such an exploration requires extensive empirical analysis. It is however, not practically possible to experiment on all the infinite distributions that exist. Therefore, the analysis needs to be restricted to certain family of distributions. Itay et al.~\cite{safran2017depth} provides a theoritical and empirical analysis to provide several new depth-based separation results on natural radial non-linear functions such as balls and ellipses. However, their empirical analysis is restricted to just two depth values. 

We instead seek to study the impact of hyperparameters such as width, depth and number of ensembles on generalization error in polynomial function approximation. One study~\cite{lawrence1998size} similarly attempted to investigate empricial performance of neural networks on polynomials while varying the hyperparameters. However, this analysis was constrained to a constant depth of 2 and limited width of 50.  \\

There are also other theories and attempts regarding empirical investigation of network hyperparameters on generalization errors in approximating polynomials but these studies are limited as they haven't considered the simultaneous possibility of variations in all the dimensions including: width, depth and number of ensembles. 

%%%%
% Malach, Eran, and Shai Shalev-Shwartz. "Is deeper better only when shallow is good?." *arXiv preprint arXiv:1903.03488* (2019).\\

% •  They Give a depth separation argument for distributions with fractal structure (A fractal is a never-ending pattern), showing that they can be expressed efficiently by deep networks, but not with shallow ones. \\
% • The success of learning deep networks depends on whether the distribution can be well approximated by shallower networks, \\
% • They show (empirically) that when training on such distributions, a clear depth separation is observed, and deeper networks indeed perform better than shallow networks. \\

% \textbf{Caveats}: \\
% • Question on the performance of deep networks in scenarios where shallow ones doesn't perform better.  \\
% • No theoretical evidence to support their claim. Their reason is that analysis of gradient-descent on deep networks proves to be extremely hard due to the dynamics of the non-convex optimization.\\

% Pei, Jin-Song, Joseph P. Wright, and Andrew W. Smyth. "Mapping polynomial fitting into feedforward neural networks for modeling nonlinear dynamic systems and beyond." *Computer Methods in Applied Mechanics and Engineering* 194.42-44 (2005): 4481-4505.\\

% Emschwiller, Matt, et al. "Neural networks and polynomial regression. demystifying the over-parametrization phenomena." *arXiv preprint arXiv:2003.10523* (2020).\\

% • Their study focuses on Overparametrization (phenom-ena whereby these models appear to generalize well on the unseen data, even though the number of parameters significantly exceeds the sample sizes) vs Generalization
% • Using Teacher/Student model approach, where the teacher model is approximated by a student to achieve a comparable performance.  \\

% \textbf{Caveats}:
% • They don't work on approximating directly the polynomial, instead they focus on tensor regression coefficients obtained from polynomial regression models. \\
% • Their focus of paramaterization is only on regression coefficients and depth.\\

% Lawrence et al., “What Size Neural Network Gives Optimal Generalization? Convergence Properties of Backpropagation”, Technical Report, 1996 \\

% * The main focus in most these papers is that deep networks have the theoretical guarantees which shallow networks do not have in terms of theoritical approximation. Generalizability (in terms of performance in unseen data-points) is a key issue that has not been addressed, since, it requires a complete empirical analysis (generalization bounds and results in general, depends on the data distribution). Works considering approximation of polynomials (we know so far) haven't considered the simultaneous possibility of variations in all the dimensions including: width, depth and number of ensembles.\\
